On the Battery Consumption of Mobile Browsers

Mobile web browsing has recently surpassed desktop browsing both in term of popularity and traffic. Following its desktop counterpart, the mobile browsers ecosystem has been growing from few browsers (Chrome, Firefox, and Safari) to a plethora of browsers, each with unique characteristics (battery friendly, privacy preserving, lightweight, etc.). In this paper, we introduce a browser benchmarking pipeline for Android browsers encompassing automation, in-depth experimentation, and result analysis. We tested 15 Android browsers, using Cappuccino a novel testing suite we built for third party Android applications. We perform a battery-centric analysis of such browsers and show that: 1) popular browsers tend also to consume the most, 2) adblocking produces significant battery savings (between 20 and 40% depending on the browser), and 3) dark mode offers an extra 10% battery savings on AMOLED screens. We exploit this observation to build AttentionDim, a screen dimming mechanism driven by browser events. Via integration with the Brave browser and 10 volunteers, we show potential battery savings up to 30%, on both devices with AMOLED and LCD screens.

==> sections/automate-io.tex <==
 % \begin{figure*}[htb]
 %     \centering
 %        \subfigure[\webtool experiment status GUI.]{\psfig{figure=\folder/remote-access, width=2in}\label{fig:visual-remote}}
 %        \subfigure[\webtool analytics reporting.]{\psfig{figure=\folder/analytics, width=2in}\label{fig:visual-analytics}}
 %        \subfigure[\webtool mturk integration.]{\psfig{figure=\folder/mturk-test, width=2in}\label{fig:visual-mturk}}
 %        % \subfigure[CDF of battery discharge across Alexa's top 1,000 websites ; Brave vs Chrome ; 5 devices and 3 network locations (UK, NJ, IL)]{\psfig{figure=\folder/placeholder, width=2.1in}\label{fig:res-c}}        
 %        % \caption{--}
 %     \label{fig:res}
 % \end{figure*}

% As a next step, we examine the best and worst performing websites with respect to power consumption (Table~\ref{tab:wpm_summ}) and compare their performance using a single \tool location (SM-J337A, New Jersey) and different Android browsers (Chrome, Firefox, Opera, and Brave). \mvnote{TODO}

% \begin{table}[tb]
% \small
% \centering
% \begin{tabular}{rccccc}
% \hline
%     {\bf URL}   & {\bf Brave} & {\bf Chrome} & {\bf Firefox} & {\bf Opera} \\
% \hline
%     arescadon.com        & 20.2  & 22    & -  & -  \\ 
%     parronnotandone.info & 20.2  & 20.8  & -  & -  \\
%     investreviewier.com  & 20.4  & 21.8  & -  & -  \\
%     maranhesduve.club    & 20.4  & 22.2  & -  & -  \\
%     2ch.net              & 20.4  & 22.3  & -  & -  \\
%     ...\\
%     ensonhaber.com       & 36.5  & 29.86 & -  & - \\  
%     nicovideo.jp         & 36.9  & 30.23 & -  & - \\
%     bulbagarden.net      & 37.2  & -     & -  & - \\
%     vnexpress.net        & 38.4  & 29.2  & -  & - \\
%     aol.com              & 41.4  & 27.96 & -  & - \\
% \end{tabular}
% \caption{Top and bottom 5 websites in term of energy consumption ; SM-J337A (NJ); Brave, Chrome, Firefox, Opera} 
% %\vspace{-0.1in}
% \label{tab:wpm_summ}
% %\vspace{-0.1in}
% \end{table}


%We opened up \webtool to the public on November 2019 and since then XX websites were tested by random visitors. Results from these tests are available at \url{https://batterylab.dev/website-stats.html}.








==> sections/data_collection.tex <==
\begin{table*}[t]
%\small
\centering
\begin{tabular}{rcccccc}
\hline

           {\bf Browser}  & {\bf Version} & {\bf Chrome/Firefox Vrs} & {\bf Popularity~\footnote{Combined popularity between MacOS/Windows (Desktop) and iOS/Android (Mobile) as reported in~\cite{browser_share} as of February 2019. When not available, we offer the number of downloads from Google Play Store - \mvnote{can we check iOS data too?}}} & {\bf Adblocking} & {\bf Dark Mode} &  {\bf Power Saving Mode}\\
\hline
{\bf Chrome}         & 72.0.3626.96  & 72.0.3626.96 & 64\%      & - & - & - \\
{\bf Baidu}          & 72.0.3626.96  & 72.0.3626.96 & 2.17\%    & - & - & - \\
{\bf UC-browser}     & 72.0.3626.96  & 72.0.3626.96 & 2.01\%    & - & - & - \\
{\bf QQ}             & 72.0.3626.96  & 72.0.3626.96 & 1.52\%    & - & - & - \\
{\bf Firefox}        & 72.0.3626.96  & 72.0.3626.96 & 0.36\%    & Addons & - & - \\
{\bf Adblock-browser}& 72.0.3626.96  & 72.0.3626.96 & >10M      & Native & - & - \\
{\bf Brave}          & 72.0.3626.96  & 72.0.3626.96 & >10M      & Native & - & - \\
{\bf Firefox-focus}  & 72.0.3626.96  & 72.0.3626.96 & >5M       & Native & - & - \\
{\bf Kiwi}           & 72.0.3626.96  & 72.0.3626.96 & >500k     & Native & - & - \\
{\bf Chrome}         & 72.0.3626.96  & 72.0.3626.96 & 64\%      & - & - & - \\
{\bf Baidu}          & 72.0.3626.96  & 72.0.3626.96 & 2.17\%    & - & - & - \\
{\bf UC-browser}     & 72.0.3626.96  & 72.0.3626.96 & 2.01\%    & - & - & - \\
{\bf QQ}             & 72.0.3626.96  & 72.0.3626.96 & 1.52\%    & - & - & - \\
{\bf Firefox}        & 72.0.3626.96  & 72.0.3626.96 & 0.36\%    & Addons & - & - \\
{\bf Adblock-browser}& 72.0.3626.96  & 72.0.3626.96 & >10M      & Native & - & - \\
{\bf Brave}          & 72.0.3626.96  & 72.0.3626.96 & >10M      & Native & - & - \\
{\bf Firefox-focus}  & 72.0.3626.96  & 72.0.3626.96 & >5M       & Native & - & - \\
{\bf Kiwi}           & 72.0.3626.96  & 72.0.3626.96 & >500k     & Native & - & - \\
\hline
\end{tabular}
\caption{Summary of Android browser performance evaluation.}
\label{tab:summ_browser}
\end{table*}
%AdBlock Plus/uBlock Origin

%%%%%%%%%%%%%%%%%%%%%%
\section{Data Collection}
\label{sec:meth}
%%%%%%%%%%%%%%%%%%%%%%
In this section we describe how we leverage \pipe to collect, at scale, battery consumption of \numbrowser Android browsers. First, we discuss the browser selection process. Next, we focus on the \emph{workloads} selection, \ie target websites to be browsed and how.  

%\blab currently consists of three vantage points, two in the US and one in Europe and hosts a range of Android devices and an iOS device (iPhone~7). A centralized server is used to deploy \emph{jobs}, \eg scripts for testing a target application. \blab offers very simple APIs to \textit{prepare} a device for testing, \eg pause notification and kill potential background processes, and automate the actual battery readings. Further, \blab grants experimenter visual access to testing devices for debugging their automation and/or record their interaction with the device. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Browser Selection}
\label{sec:meth:selection}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Our rationale for selecting browsers to test is threefold. First, we want to test \emph{popular} browsers since representative of which browsers run in the wild. Second, we want to test \emph{adblocking} browsers -- either native or enahnced with adblocking addons -- because of the potential energy benefits associated with adblocking~\cite{}. Finally, we want to test browsers which advertise energy saving capabilites. 

Based on the above strategy, Table\ref{tab:summ_browsers} summarizes which browsers have been selected along with general information and motivation for selection. Overall, we will be testing \numandroid Android and \numios iOS browsers. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Workload Selection}
\label{sec:meth:workload}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
While existing studies focus on arbitrary set of websites to test, we here propose several workloads that cover a large set of user interactions with a browser. In the selection of our workloads, we make sure that the pages select do not contain consent elements, like for cookies or tracking (GDPR). Such consent elements need to be clicked in order to allow for the full content to be displayed which can impact the results, especially when studying adblocking performance. However, intercepting and clicking such elements across the set of browsers we are studying is quite challenging. 

\vspace{0.1in}
\noindent \textbf{Cold Start}   -- This is the simplest of the workload where we just launch a browser to its home and wait for 60 seconds. The goal of this workload is to gain insights on the bottom line energy consumption of a browser regardless of the content being displayed. 

\vspace{0.1in}
\noindent \textbf{Tab Monster}  -- In this workload, we vary the number of concurrent tabs opened in the browser. Since the number of tabs rather than the displayed content is of interest in this workload, we simply use as input Alexa's top 100 pages -- yes, we stress test each browser up to 100 tabs. 

\vspace{0.1in}
\noindent \textbf{Popular News} -- In this workload, we sequentially load the landing page of  the ten most popular news website. We chose news websites since they are typical destination especially for mobile users. We chose 10 websites to a) keep the experiment duration reasonable in time, b) 10 is a typical number of concurrent tabs a user would open~\cite{concurrent_tabs}. 

\vspace{0.1in}
\noindent \textbf{Ads Free} -- This workload consists of 10 popular websites with no or minimal advertisement.  The goal of this workload is to offer a worst case scenario for browsers focusing on adblocking. For our selection, we crawled Alexa's top 1,000 websites and run them through a local adblocker to identify presence of lack of advertisement. Next, we select the top 10 websites with minimal advertisements which do not contain consent elements. 

Independently of the workload, we automate a page load as follows. The target page is requested and $T$ seconds are allowed to load.\footnote{While Chromium based browsers on Android can offer page load time information, this approach would not be generic across browsers}. Next, we simulate multiple user interactions by scrolling the page up and down multiple times. 

==> sections/power-saving.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Power Saving Evaluation}
\label{sec:power}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we report performance comparison (CPU, bandwidth, battery) of two broad browser categories: adblocking and power saving browsers. 

%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Adblocking}
\label{sec:power:adblocking}
%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[thb]
   \centering
   \subfigure[Energy]{\psfig{figure=\folder/adblocking-discharge-comparison, width=2.1in}\label{fig:res:vanilla_discharge}}
   \subfigure[Bandwidth.]{\psfig{figure=\folder/adblocking-bdw-comparison, width=2.1in}  \label{fig:res:vanilla_bdw}}           
   \subfigure[CPU.]{\psfig{figure=\folder/adblocking-cpu-comparison, width=2.1in}    \label{fig:res:vanilla_cpu}}      
   \caption{Performance comparison of adblocking browsers.} 
   \label{fig:results_adblocking_vanilla}
 \end{figure*}


We here compare Brave’s battery consumption against several adblocking  Android browsers: Adblock (1.4.0), Kiwi (Eta), Firefox (65.0) equipped with the ublock plugin (vrs 1.18.4), and Firefox-focus (8.0.6).  The left plot shows that Adblock, Kiwi, and Firefox-focus achieves a similar average battery discharge (90-100mAh) which is a 20\% reduction compared to regular non-adblocking browsers. Brave further reduces battery consumption by 20\%, with average discharge around 80mAh as previously reported. While Firefox-ublock seems more competitive (90mAh, on average), it should not be forgotten that Firefox leverages the advantage of lacking page interaction which we estimated at an extra 15mAh.

As above, the right plot shows that Brave’s battery savings derive from a combination of “browser” and “android” savings. Differently from above, battery-historian overestimation does not hold for all browsers making Kiwi the closest competitor to Brave (according to this tool). 


Adblocking browsers are expected to have an overall lower bandwidth consumption compared to vanilla browsers. With the exception of Kiwi, this is indeed the case and all browsers have a similar bandwidth footprint. Brave is still by far the least CPU-hungry browser (20-40\% reduction), even more efficient than Firefox without webpage interaction. In presence of a similar network footprint, these CPU savings are responsible of the above battery savings.

\begin{figure*}[thb]
   \centering
   \subfigure[DarkMode]{\psfig{figure=\folder/dark-mode.png, width=2.1in}\label{fig:res:darkmode}}
   \subfigure[]{\psfig{figure=\folder/placeholder, width=2.1in}  \label{fig:res:a}} 
   \subfigure[]{\psfig{figure=\folder/placeholder, width=2.1in} \label{fig:res:b}}      
   \caption{Performance comparison of (populr) power saving modes.}
   \label{fig:results_power_saving}
 \end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Darkreading}
\label{sec:power:darkreading}
%%%%%%%%%%%%%%%%%%%%%%%%%%


Brave/Chrome dark mode - 7\% savings 

Kiwi night mode - 16\% savings


%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ad-hoc}
\label{sec:power:adhoc}
%%%%%%%%%%%%%%%%%%%%%%%%%%
